SVGDreamer++: Advancing Editability and Diversity in Text-Guided SVG Generation

Recently, text-guided scalable vector graphics (SVG) synthesis has demonstrated significant potential in domains such as iconography and sketching. However, SVGs generated from existing Text-to-SVG methods often lack editability and exhibit deficiencies in visual quality and diversity. In this paper, we propose a novel text-guided vector graphics synthesis method to address these limitations. To enhance the editability of output SVGs, we introduce a Hierarchical Image VEctorization (HIVE) framework that operates at the semantic object level and supervises the optimization of components within the vector object. This approach facilitates the decoupling of vector graphics into distinct objects and component levels. Our proposed HIVE algorithm, informed by image segmentation priors, not only ensures a more precise representation of vector graphics but also enables fine-grained editing capabilities within vector objects. To improve the diversity of output SVGs, we present a Vectorized Particle-based Score Distillation (VPSD) approach. VPSD addresses over-saturation issues in existing methods and enhances sample diversity. A pre-trained reward model is incorporated to re-weight vector particles, improving aesthetic appeal and enabling faster convergence. Additionally, we design a novel adaptive vector primitives control strategy, which allows for the dynamic adjustment of the number of primitives, thereby enhancing the presentation of graphic details. Extensive experiments validate the effectiveness of the proposed method, demonstrating its superiority over baseline methods in terms of editability, visual quality, and diversity. We also show that our new method supports up to six distinct vector styles, capable of generating high-quality vector assets suitable for stylized vector design and poster design. Code and demo will be released at: http://ximinng.github.io/SVGDreamerV2Project/

==> sec/0_abstract_bk.tex <==
\begin{abstract}
Recently, text-guided scalable vector graphics (SVGs) synthesis has demonstrated significant potential in domains such as iconography and sketch. 
However, SVGs generated from existing text-to-SVG methods often lack editability and exhibit deficiencies in visual quality and diversity. 
To address these limitations, we propose a novel text-guided vector graphics synthesis method termed SVGDreamer++.
%SVGDreamer incorporates a semantic-driven image vectorization (SIVE) process that enables the decomposition of synthesis into foreground objects and background, thereby enhancing editability.
SVGDreamer++ has two essential components. The first is the fine-grained image vectorization scheme (FIVE) which is designed to improve editabilty. FIVE is built upon a novel semantic-driven image vectorization (SIVE) process that enables the decomposition of synthesis into foreground objects and background. 
SIVE leverages attention priors to supervise SVG reconstruction for a decoupled representation of vector graphics.
FIVE improve the editbility  further by incorporating image segmentation priors to realize part-level manipulation for SVG generation.
%Moreover, to further control and manipulate the local composition of the elements in the SVG, we propose a fine-grained image vectorization scheme (FIVE).
%FIVE introduces image segmentation priors to supervise SVG reconstruction, achieving an accurate representation of the vector graphic.
Moreover, 
a novel adaptive vector primitives control technique is proposed to enhance graphic details.
We also present a Vectorized Particle-based Score Distillation (VPSD) approach to tackle over-saturation issues, enhance sample diversity, and utilizes a pre-trained reward model to re-weight vector particles for improved aesthetic appeal and faster convergence.
%SVGDreamer also proposes a Vectorized Particle-based Score Distillation (VPSD) approach to tackle over-saturation issues, enhance sample diversity, and utilizes a pre-trained reward model to re-weight vector particles for improved aesthetic appeal and faster convergence.
Extensive experiments are conducted to validate the effectiveness of SVGDreamer++, demonstrating its superiority over baseline methods in terms of editability, visual quality, and diversity.
%Furthermore, we demonstrate the applicability of our approach in vector design, including icon and poster design.
SVGDreamer++ supports up to six distinct vector styles, and our experiments indicate that it can generate high-quality vector assets suitable for stylized vector design. We also show its applicability in vector design, such as icon and poster design.
\end{abstract}

\begin{IEEEkeywords}
Vector Graphics, SVG Generation, Vectorization, Text-to-SVG
\end{IEEEkeywords}

==> sec/6_biography.tex <==
\section{Biography Section}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{profile/xxm.jpg}}]{Ximing Xing} is currently pursuing the Ph.D. degree with the school of software from Beihang University, China. His research interests include deep generation, vector graphics generation, diffusion models, and the combination of art and technology. His works have been published in top-tier conferences, such as NeurIPS and CVPR.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{profile/yq.jpg}}]{Qian Yu} received her Ph.D. degree from Queen Mary University of London, UK, in 2018. From 2018 to 2019, she was a post-doctoral researcher at UC Berkeley. She is now an associate professor at Beihang University. She was a coauthor of a paper that won the Best Paper Award at the British Machine Vision Conference (BMVC) in 2015. Her research interests include computer vision and deep learning, with special interests in sketch understanding and applications.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{profile/chuangwang.jpg}}]{Chuang Wang} received the BE. degree from Beihang University, China, in 2023. He is currently pursuing the master's degree with Beihang University. His current research interests include sketch generation, video generation and multi-modal deep learning tasks.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{profile/zht.png}}]{Haitao Zhou} received the B.E. degree from Beihang University, China, in 2023. He is currently pursuing the master's degree with Beihang University. His current research interests include sketch generations and video generations.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{profile/zhangjing.png}}]{Jing Zhang} received her Ph.D. degree from University of Wollongong, Australia, in 2019. She is now an associate professor in School of Software, Beihang University, Beijing, China. Her recent research interests include machine learning and computer vision, with the special interests in transfer learning, multi-modality learning, open-vocabulary learning, and their applications in data-efficient computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{profile/dongxu.jpeg}}]{Dong Xu (Fellow, IEEE)} received the B.E. and Ph.D. degrees from the University of Science and Technology of China, Hefei, China, in 2001 and 2005, respectively. While pursuing the Ph.D. degree, he was an Intern with Microsoft Research Asia, Beijing, China, and a Research Assistant with The Chinese University of Hong Kong, Hong Kong, for more than two years. He was a Post-Doctoral Research Scientist with Columbia University, New York, NY, USA, for one year. He also worked as a Faculty Member at Nanyang Technological University, Singapore, and the Chair of computer engineering at The University of Sydney, Camperdown, NSW, Australia. He is currently a Professor with the Department of Computer Science, The University of Hong Kong, Hong Kong. He was a coauthor of a paper that won the Best Student Paper Award at the IEEE Conference on Computer Vision and Pattern Recognition (CVPR) in 2010 and a paper that won the Prize Paper award in IEEE TRANSACTIONS ON MULTIMEDIA (T-MM) in 2014. His current research interests include computer vision, statistical learning, and multimedia content analysis.
\end{IEEEbiography}

\vfill
